Smart Greybox Fuzzing

Coverage-based greybox fuzzing (CGF) is one of the most successful methods for automated vulnerability detection. Given a seed file (as a sequence of bits), CGF randomly flips, deletes or bits to generate new files. CGF iteratively constructs (and fuzzes) a seed corpus by retaining those generated files which enhance coverage. However, random bitflips are unlikely to produce valid files (or valid chunks in files), for applications processing complex file formats. In this work, we introduce smart greybox fuzzing (SGF) which leverages a high-level structural representation of the seed file to generate new files. We define innovative mutation operators that work on the virtual file structure rather than on the bit level which allows SGF to explore completely new input domains while maintaining file validity. We introduce a novel validity-based power schedule that enables SGF to spend more time generating files that are more likely to pass the parsing stage of the program, which can expose vulnerabilities much deeper in the processing logic. Our evaluation demonstrates the effectiveness of SGF. On several libraries that parse structurally complex files, our tool AFLSmart explores substantially more paths (up to 200%) and exposes more vulnerabilities than baseline AFL. Our tool AFLSmart has discovered 42 zero-day vulnerabilities in widely-used, well-tested tools and libraries; so far 17 CVEs were assigned.

==> sections-tse/case.tex <==
\section{Case Study: Discovered Bugs}
\label{sec:case}
In this section, we have a closer look at some of the zero-day vulnerabilities that \smart has discovered in WavPack and FFmpeg. We investigate how much the input-structure-awareness of \smart contributed to the discovery of the vulnerabilities in terms of  a qualitative analysis.

\subsection{WavPack}
\smart discovered five vulnerabilities in WavPack (CVE-[blinded-1] through CVE-[blinded-5]). In \ref{sec:motivating}, we discussed how \smart's capabilities of fuzzing the file structure rather than the file's bits led to 
the discovery of  CVE-[blinded-1] and CVE-[blinded-2].

In the following, we discuss another CVE (CVE-[blinded-3]) that \smart discovered in WavPack. The \emph{buffer overwrite} is caused by two integer overflows and insufficient memory allocation. To construct an exploit, we need to craft a \emph{valid WAVE file} that contains the mandatory \texttt{riff}, \texttt{fmt}, and \texttt{data} chunks. Between the \texttt{fmt} and \texttt{data} chunk, we add an \emph{additional unknown chunk} (i.e., that is neither fmt, data, ..) with \texttt{cksize} $ \ge 0\text{x}80000000$.

\begin{figure}[h]
\begin{tabular}{@{}l@{\quad}l}
%\multicolumn{2}{@{}l}{Showing \texttt{cli/riff.c} @ revision \texttt{0a72951}}\\
\tiny{286}&\small \texttt{\textbf{else} \{}\quad\quad\quad\quad\quad\quad\emph{// just copy unknown chunks to output file}\\
\tiny{287}&\\
\tiny{288}&\small \texttt{\quad \textbf{int} bytes\_to\_copy = (chunk\_header.ckSize + 1) \& ~1L;}\\
\tiny{289}&\small \texttt{\quad \textbf{char} *buff = malloc (bytes\_to\_copy);}\\
\ldots\\
\tiny{296}&\small \texttt{\quad \textbf{if} (!DoReadFile (infile, buff, bytes\_to\_copy,..)) \{}\\
\end{tabular}
\caption{Showing \texttt{cli/riff.c} @ revision \texttt{0a72951}}
\label{fig:vuln1}
\end{figure} 

During parsing the file, WavPack enters the ``unknown chunk'' handling code shown in \ref{fig:vuln1}. It reads the specified chunk size from the \texttt{chunk\_header} struct and stores it as a 32-bit \emph{signed} integer. Since \texttt{ckSize} $ \ge 2^{31}$, the assignment in \texttt{riff.c:288} overflows, such that \texttt{bytes\_to\_copy} contains a negative value. The memory allocation function \texttt{malloc} takes only unsigned values causing a second overflow to a smaller positive number. When \texttt{DoReadFile} attempts to read more information from the WAVE file, there is not enough memory being allocated, resulting in a memory overwrite that can be controlled by the attacker.
%
This vulnerability (CVE-[blinded-3]) was patched by aborting when \texttt{bytes\_to\_copy} is negative.

\subsection{FFmpeg}
\smart discovered a crashing bug in FFmpeg, a widely used library for encoding and decoding audio and video files. The crash is caused by a division by zero. In order to reproduce the crash, an attacker must craft a Audio Video Interleave (AVI) file which has at least one audio stream where the sample rate is set to zero. The AVI file contains the mandatory \texttt{hdrl} (header list) and \texttt{movi} chunks. The \texttt{hdrl} chunk contains at least one \texttt{strl} (stream header list) chunk which itself contains the mandatory \texttt{strh} (stream header), \texttt{strf} (stream format), and \texttt{index} chunks. The \texttt{strh} chunk uses the WAVEFORMATEX structure to specify 0 for attribute \texttt{wBitsPerSample} while passing all other sanity checks.

The code in FFmpeg that processes the information stored in the crafted AVI file does not check for the sample rate to be zero when it computes the next decoding time stamp (next\_dts; see \ref{fig:vuln3}).

\begin{figure}[h]
\begin{tabular}{@{}l@{\quad}l}
%\multicolumn{2}{@{}l}{Showing \texttt{cli/riff.c} @ revision \texttt{0a72951}}\\
\tiny{2712}&\small \texttt{\textbf{case} AVMEDIA\_TYPE\_AUDIO:}\\
\tiny{2713}&\small \texttt{\quad ist->next\_dts += ((int64\_t)AV\_TIME\_BASE *}\\
&\small \texttt{\quad\quad\quad\quad ist->dec\_ctx->frame\_size) /}\\
\tiny{2714}&\small \texttt{\quad\quad\quad ist->dec\_ctx->sample\_rate;}
\end{tabular}
\caption{Showing \texttt{fftools/ffmpeg.c} @ revision \texttt{a150b2e}}
\label{fig:vuln3}
\end{figure} 
The crashing bug was fixed\footnote{\url{https://patchwork.ffmpeg.org/patch/[blinded]/}} by introducing a check whether the sample rate is zero. If it is, the next decoding time stamp is computed by rescaling.



==> sections-tse/guideline.tex <==
\hfill

This is a guideline to quickly write \smart -compatible file format specifications based on the Peach Pit schema \cite{peach18}. Before going into the detailed steps, the following are our general rules of thumb:

\begin{itemize}[itemsep=0.1cm]
  \item \emph{Rule-1. Chunk inheritance}. Most file formats are composed of data chunks which normally share a common structure. Like an abstract class in Java, we start by modelling a generic chunk containing attributes that are shared across all chunks in the file format. Then, we model the concrete chunks which inherit the attributes from the generic chunk. Hence, we only need to insert/modify chunk-specific attributes.
  \item \emph{Rule-2. Model completeness}. As explained in \ref{sec:grammar}, \smart applies structural mutation operators that work at chunk level. So we are not required to specify all attributes inside a chunk. We can start with some coarse-grained model and gradually make it more complete.
  \item \emph{Rule-3. Relaxed constraints}. There could be many constraints in a chunk (e.g., the chunk identifier must be a constant string, the chunk size attribute must match with the actual size or chunks must be in order). However, since the main goal of fuzzing or stress testing in general is to explore corner cases, we should relax some constraints as long as these relaxed constraints do not prevent the parser from decomposing the file.
\end{itemize}

\hfill

Following are the three steps for developing a Peach Pit file format specification. We use WAVE file format from our motivating example in \ref{sec:motivating} to illustrate each step.

\subsection*{Step 1. Understanding the File Format}
%
It is not necessary for a Peach Pit to specify the full file format in order to be useful for \smart. Instead a coarse format specification is perfectly sufficient. 
%We do not need to read the whole official file format specification, which could be thousand-page long, to understand the high level structure of a given file format. We could easily find more concise technical documents, blog posts or Wikipedia pages which summarize the file structure. 
As an example, this Wikipedia page \cite{wavformat} has all basic information of the WAVE file format. A WAVE starts with some header information (RIFF and WAVE tokens) followed by several chunks while each chunk has specific chunk identifier, chunk length and data (cf. \ref{tab:wave}).

\subsection*{Step 2. Validate Our Understanding}
\begin{figure}[h]
\includegraphics[width=\columnwidth]{figures/010editor}
\caption{Analyzing file structures using 010Editor}
\label{fig:editor}
\end{figure}

We can use a Hex editor tool  called 010Editor \cite{editor010} to analyze sample files to validate our understanding. The tool is very handy and supports so-called ``templates'' to parse and decompose a given input file into chunks and attributes. The tool currently provides 114 such templates for the most common file formats \cite{templates010}.
%
\ref{fig:editor} is a screenshot of 010Editor displaying a WAVE file. The top part of the screen shows the raw data in both Hexadecimal and ASCII modes. The bottom part is the decomposed data. We can see the WAVE file header, its format chunk, data chunk and so on.

\subsection*{Step 3. Develop the Peach Pit}

Peach provides a very comprehensive tutorial\footnote{http://community.peachfuzzer.com/v3/PeachQuickStart.html}; please refer to this  for learning its basic concepts like Data Model, Block, Choice, token, Relation and so on.

Rule-1 states that we should leverage the chunk inheritance. As all chunks have chunk identifier, chunk length and chunk data, we first design a model for a generic chunk as shown in Listing~\ref{lst:wavegeneric}.

\hfill 

\lstset{%
   		framexleftmargin=0mm,
   		frame=single,
   		numbers=none,
		resetmargins=true,
   		%numberstyle=\tiny,
   %		commentstyle=\metaTextStyle\small,
   		basicstyle=\ttfamily\selectfont\footnotesize,
   	  frameround= tttt,
   	  breaklines = true,
   	  tabsize=1,
   	  captionpos=b,
   	  language=C,
   	  morekeywords={Bug}}
\begin{lstlisting}[frame=single, caption=Generic Chunk Model, label=lst:wavegeneric]
<DataModel name="Chunk">
 <String name="ckID" length="4" padCharacter=" "/>
 <Number name="cksize" size="32">
  <Relation type="size" of="Data"/>
 </Number>
 <Blob name="Data"/>
 <Padding alignment="16"/>
</DataModel>
\end{lstlisting}

%\hfill

Once the generic chunk has been defined, we can model other chunks based on this generic chunk. As other chunk share the same structure as the generic chunk, we only need to specifiy chunk-specific attributes. \ref{lst:wavefmt} shows the definition for a format chunk.

\vfill

\lstset{%
   		framexleftmargin=0mm,
   		frame=single,
   		numbers=none,
		resetmargins=true,
   		%numberstyle=\tiny,
   %		commentstyle=\metaTextStyle\small,
   		basicstyle=\ttfamily\selectfont\footnotesize,
   	  frameround= tttt,
   	  breaklines = true,
   	  tabsize=1,
   	  captionpos=b,
   	  language=C,
   	  morekeywords={Bug}}
\begin{lstlisting}[frame=single, caption=Format Chunk Model, label=lst:wavefmt]
<DataModel name="ChunkFmt" ref="Chunk">
   <String name="ckID" value="fmt "  token="true"/>
   <Block name="Data">
      <Number name="wFormatTag" size="16"/>
      <Number name="nChannels" size="16"/>
      <Number name="nSampleRate" size="32"/>
      <Number name="nAvgBytesPerSec" size="32"/>
      <Number name="nBlockAlign" size="16" />
      <Number name="nBitsPerSample" size="16"/>
   </Block>
</DataModel>
\end{lstlisting}

\hfill


Rule-2 states that we are not required to specify all attributes of a chunk. \ref{lst:wavefmtsimple} shows a simplified definition of the format chunk in which we only specify the chunk identifier. Note that, if the token property of the \emph{ckID} attribute is set to true, it means that Peach only identifies format chunk(s) having the exact value of "fmt ".

\hfill

\lstset{%
   		framexleftmargin=0mm,
   		frame=single,
   		numbers=none,
		resetmargins=true,
   		%numberstyle=\tiny,
   %		commentstyle=\metaTextStyle\small,
   		basicstyle=\ttfamily\selectfont\footnotesize,
   	  frameround= tttt,
   	  breaklines = true,
   	  tabsize=1,
   	  captionpos=b,
   	  language=C,
   	  morekeywords={Bug}}
\begin{lstlisting}[frame=single, caption=Simplified Format Chunk Model, label=lst:wavefmtsimple]
<DataModel name="ChunkFmt" ref="Chunk">
   <String name="ckID" value="fmt "  token="true"/>
</DataModel>
\end{lstlisting}

Similarly, we can define the models for other chunks such as Data chunk, Fact chunk, Wavl chunk and so on. Once all chunks have been defined, we can model the whole WAVE file itself as a big data model. 
\ref{lst:wavfull} shows the definition of a WAVE file. Rule-3 states that we should relax some constraints to explore more corner cases. As we use the \emph{Choice} element to specify the list of potential chunks (including both mandatory and optional ones), many constraints have been relaxed. First, the chunks can appear in a different order. Secondly, some chunk (including mandatory chunk) can be absent. Thirdly, some unknown chunk can appear. Lastly, some chunk can appear more than once. In fact, due to this relaxed model, vulnerabilities like the one in our motivating example in our paper (Section \ref{sec:motivating}) can be exposed.

\lstset{%
   		framexleftmargin=0mm,
   		frame=single,
   		numbers=none,
		resetmargins=true,
   		%numberstyle=\tiny,
   %		commentstyle=\metaTextStyle\small,
   		basicstyle=\ttfamily\selectfont\footnotesize,
   	  frameround= tttt,
   	  breaklines = true,
   	  tabsize=1,
   	  captionpos=b,
   	  language=C,
   	  morekeywords={Bug}}
\begin{lstlisting}[frame=single, caption=WAVE Peach Pit File Format Specification, label=lst:wavfull]
<DataModel name="Wav">
  <String name="ckID" value="RIFF" token="true"/>
  <Number name="cksize" size="32" />
  <String name="WAVE" value="WAVE" token="true"/>
  <Choice name="Chunks" maxOccurs="30000">
    <Block name="FmtChunk" ref="ChunkFmt"/>
    <Block name="DataChunk" ref="ChunkData"/>
    <Block name="FactChunk" ref="ChunkFact"/>
    <Block name="SintChunk" ref="ChunkSint"/>
    <Block name="WavlChunk" ref="ChunkWavl"/>
    <Block name="CueChunk" ref="ChunkCue"/>
    <Block name="PlstChunk" ref="ChunkPlst"/>
    <Block name="LtxtChunk" ref="ChunkLtxt"/>
    <Block name="SmplChunk" ref="ChunkSmpl"/>
    <Block name="InstChunk" ref="ChunkInst"/>
    <Block name="OtherChunk" ref="Chunk"/>
  </Choice>
</DataModel>
\end{lstlisting}





